Modeling the Sequential Dependence among Audience Multi-step Conversions with Multi-task Learning in Targeted Display Advertising

In most real-world large-scale online applications (e.g., e-commerce or finance), customer acquisition is usually a multi-step conversion process of audiences. For example, an impression->click->purchase process is usually performed of audiences for e-commerce platforms. However, it is more difficult to acquire customers in financial advertising (e.g., credit card advertising) than in traditional advertising. On the one hand, the audience multi-step conversion path is longer. On the other hand, the positive feedback is sparser (class imbalance) step by step, and it is difficult to obtain the final positive feedback due to the delayed feedback of activation. Multi-task learning is a typical solution in this direction. While considerable multi-task efforts have been made in this direction, a long-standing challenge is how to explicitly model the long-path sequential dependence among audience multi-step conversions for improving the end-to-end conversion. In this paper, we propose an Adaptive Information Transfer Multi-task (AITM) framework, which models the sequential dependence among audience multi-step conversions via the Adaptive Information Transfer (AIT) module. The AIT module can adaptively learn what and how much information to transfer for different conversion stages. Besides, by combining the Behavioral Expectation Calibrator in the loss function, the AITM framework can yield more accurate end-to-end conversion identification. The proposed framework is deployed in Meituan app, which utilizes it to real-timely show a banner to the audience with a high end-to-end conversion rate for Meituan Co-Branded Credit Cards. Offline experimental results on both industrial and public real-world datasets clearly demonstrate that the proposed framework achieves significantly better performance compared with state-of-the-art baselines.

==> KDD21 applied data science track/README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.75.  \country is now obligatory for addresses.
	       Added \AtBeginMaketitle

Version 1.76.  Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.77.  Changed the way to typset multiple affiliations (Christoph Sommer)

==> KDD21 applied data science track/input/conclusion.tex <==
\section{Conclusion}% and Outlook
In this paper, we proposed an Adaptive Information Transfer Multi-task (\model) framework to model the sequential dependence among audience multi-step conversions. The proposed Adaptive Information Transfer (\module) module combining the \constraint~ in the loss function could learn what and how much information to transfer for different conversion stages for improving the performance of multi-task learning with sequential dependence.
Offline and online experimental results demonstrate significant improvement compared with state-of-the-art baseline models.

% Several directions are available for future research in the area. Firstly, the Tower could be replaced with some advanced models (e.g., NFM \cite{he2017nfm}, DeepFM \cite{guo2017deepfm}, AFM \cite{xiao2017afm} and even the sequence models NHFM \cite{nhfm2020neural}, DIFM \cite{difm2021modeling}).
% Secondly, combining the \model~ and Expert-Bottom pattern-based models may bring additional gain.

\section{Acknowledgments}
Fuzhen Zhuang is supported by the National Natural Science Foundation of China under Grant Nos. U1836206, U1811461.
Besides, we thank Zhenhua Zhang, Kun Chen, Chang Qu, Qiu Xiong, and KangMing Yu for their support and valuable suggestions.


==> KDD21 applied data science track/input/experiment.tex <==
\section{Experiments}
% Table generated by Excel2LaTeX from sheet 'dataset'
\begin{table}[!t]
  \centering
  \caption{Summary statistics for the datasets. ``\%Positive'' represents the percentage of positive samples in the train set over each task.}
    \setlength{\tabcolsep}{0.6mm}{
    \begin{tabular}{cccccc}
    \toprule
    Dataset & \multicolumn{1}{l}{\#Task} & \#Train & \#Validation & \#Test & \%Positive(\%) \\
    \midrule
    Industrial & 4     & 20M   & 3M    & 26M   & 23.29/1.84/1.30/1.00 \\
    % 17.00/1.34/0.95/0.73
    Public & 2     & 38M   & 4.2M  & 43M   & 3.89/0.02 \\
    \bottomrule
    \end{tabular}
    }%
  \label{tab:dataset}%
\end{table}%
In this section, we perform experiments to evaluate the proposed framework against various baselines on both industrial and public real-world datasets.
We first introduce the datasets, evaluation protocol, and baseline methods. Finally, we present our experimental results and analysis.
% Table generated by Excel2LaTeX from sheet
\begin{table*}[!t]
  \centering
  \caption{The AUC performance (mean$\pm$std) on the industrial and public datasets. The Gain means the mean AUC improvement compared with the LightGBM. Underlined results indicate the best baselines over each task. ``*'' indicates that the improvement of the proposed \model~ is statistically significant compared with the best baselines at p-value $<$ 0.05 over paired samples t-test, and ``**'' indicates that the p-value $<$ 0.01.}
    \begin{tabular}{c|cccc|cccc}
    \toprule
    \multirow{2}[2]{*}{Model} & \multicolumn{4}{c|}{Industrial dataset} & \multicolumn{4}{c}{Public dataset} \\
          & \credit~ AUC & \activate~ AUC & \multicolumn{2}{c|}{Gain} & \click~ AUC & \purchase~ AUC & \multicolumn{2}{c}{Gain} \\
    \midrule
    LightGBM & 0.8392$\pm$0.0011 & 0.8536$\pm$0.0035 & -     & -     & 0.5837$\pm$0.0005 & 0.5870$\pm$0.0038 & -     & - \\
    MLP   & 0.8410$\pm$0.0010 & 0.8602$\pm$0.0014 & +0.0018  & +0.0066  & 0.6048$\pm$0.0013 & 0.5806$\pm$0.0035 & +0.0211  & -0.0064  \\
    \midrule
    ESMM  & 0.8443$\pm$0.0028 & 0.8691$\pm$0.0025 & +0.0051  & +0.0155  & 0.6022$\pm$0.0020 & 0.6291$\pm$0.0061 & +0.0185  & +0.0421  \\
    OMoE  & 0.8438$\pm$0.0022 & 0.8714$\pm$0.0009 & +0.0046  & +0.0178  & \textbf{\underline{0.6049$\pm$0.0020}} & 0.6405$\pm$0.0041 & \textbf{+0.0212} & +0.0535  \\
    MMoE  & 0.8444$\pm$0.0026 & 0.8705$\pm$0.0009 & +0.0052  & +0.0169  & 0.6047$\pm$0.0017 & \underline{0.6420$\pm$0.0031} & +0.0210  & +0.0550  \\
    PLE   & \underline{0.8518$\pm$0.0006} & \underline{0.8731$\pm$0.0016} & +0.0126  & +0.0195  & 0.6039$\pm$0.0014 & 0.6417$\pm$0.0013 & +0.0202  & +0.0547  \\
    AITM  & \textbf{0.8534$\pm$0.0011**} & \textbf{0.8770$\pm$0.0005*} & \textbf{+0.0142} & \textbf{+0.0234} & 0.6043$\pm$0.0016 & \textbf{0.6525$\pm$0.0024**} & +0.0206  & \textbf{+0.0655} \\
    \bottomrule
    \end{tabular}%
  \label{tab:result12}%
\end{table*}%


\subsection{Datasets}
\begin{itemize}
    \item \textbf{Industrial dataset:} The industrial dataset contains all samples that are shown a banner of Meituan Co-Branded Credit Cards over a continuous period of time. 
    We divide the training, validation, and test sets in chronological order. We downsample the \activate~ negative samples for each bank to keep the proportion of positive samples to be $1\%$ overall except for the test set. 
    Because it is necessary to evaluate the performance of the model on the test set that meets the real data distribution.
    Four tasks (i.e., \click, \apply, \credit, \activate) are contained in the dataset.
    \item \textbf{Public dataset:} The public dataset is the Ali-CCP (Alibaba Click and Conversion Prediction) \cite{esmm2018sigir} dataset\footnote{https://tianchi.aliyun.com/datalab/dataSet.html?dataId=408}. We use all the single-valued categorical features. Two tasks (i.e., \click, \purchase) are contained in the dataset. We randomly take $10\%$ of the train set as the validation set to verify the convergence of all models.
\end{itemize}
For these two datasets, we filter the features whose frequency less than 10.
The statistics of these datasets are shown in Table \ref{tab:dataset}.
\subsection{Evaluation Protocol}
In the offline experiments, to evaluate the performance of the proposed \model~framework and the baselines, we follow the existing works \cite{mmoe2018kdd,esmm2018sigir,esm22020sigir,cgc2020recsys} to use the standard metric: \textbf{AUC} (Area Under ROC).
In ranking tasks, AUC is a widely used metric to evaluate the ranking ability. The mean and  standard deviation (std) are reported over five runs with different random seeds.
In the online A/B test, we use the \textbf{end-to-end conversion rate} to evaluate the performance more intuitively.
On all datasets, we report the AUC of end-to-end tasks, which are directly optimized in their loss functions.
Besides, we only report the metrics on the focused main tasks (i.e., the \credit~and \activate~tasks) over the industrial dataset.

\subsection{Baseline Methods}
We compare the proposed method with the following competitive and mainstream models:
\begin{itemize}
    \item \textbf{LightGBM} \cite{lgb2017lightgbm}: LightGBM is a gradient boosting framework that uses tree based learning algorithms. LightGBM is being widely-used in many winning solutions of machine learning competitions\footnote{https://github.com/microsoft/LightGBM}.
    \item \textbf{MLP} \cite{gardner1998mlp}: We use the base structure of our \model~framework as the single task model. It is a Multi-Layer Perceptron.
    \item \textbf{ESMM} \cite{esmm2018sigir,esm22020sigir}: The ESMM and $ESM^2$ with Probability-Transfer pattern are designed for solving the non-end-to-end post-click conversion rate via training on the entire space to relieve the sample selection bias problem.
    \item \textbf{OMoE} \cite{mmoe2018kdd}: The OMoE with Expert-Bottom pattern integrates experts via sharing one gate among all tasks.
    \item \textbf{MMoE} \cite{mmoe2018kdd}: The MMoE with Expert-Bottom pattern is designed to integrate experts via multiple gates in the Gate Control as shown in Figure \ref{fig:model} (a).
    \item \textbf{PLE} \cite{cgc2020recsys}: The Progressive Layered Extraction (PLE) with Expert-Bottom pattern separates task-shared experts and task-specific experts explicitly. This is the state-of-the-art method under different task correlations.
\end{itemize}

\subsection{Performance Comparison}
\subsubsection{\textbf{Offline Results}}
% % Table generated by Excel2LaTeX
% \begin{table}[!t]
%   \centering
%   \caption{The AUC performance (mean$\pm$std) on the industrial dataset. The Gain means the mean AUC improvement compared with the LightGBM. Underlined results indicate the best baselines over each task. ``*'' indicates that the improvement of the proposed \model~ is statistically significant compared with the best baselines at p-value $<$ 0.05 over paired samples t-test, and ``**'' indicates that the p-value $<$ 0.01.}
%   \vspace{-0.3cm}
%     \setlength{\tabcolsep}{0.82mm}{
%     \begin{tabular}{cllll}
%     \toprule
%     Model & \credit~ AUC & \activate~ AUC & \multicolumn{2}{c}{Gain} \\
%     \midrule
%     LightGBM & 0.8392$\pm$0.0011 & 0.8536$\pm$0.0035 & -     & - \\
%     MLP   & 0.8410$\pm$0.0010 & 0.8602$\pm$0.0014 & +0.0018  & +0.0066  \\
%     \midrule
%     ESMM  & 0.8443$\pm$0.0028 & 0.8691$\pm$0.0025 & +0.0051  & +0.0155  \\
%     OMoE  & 0.8438$\pm$0.0022 & 0.8714$\pm$0.0009 & +0.0046  & +0.0178  \\
%     MMoE  & 0.8444$\pm$0.0026 & 0.8705$\pm$0.0009 & +0.0052  & +0.0169  \\
%     PLE   & \underline{0.8518$\pm$0.0006} & \underline{0.8731$\pm$0.0016} & +0.0126 & +0.0195 \\
%     AITM  & \textbf{0.8534$\pm$0.0011**} & \textbf{0.8770$\pm$0.0005*} & \textbf{+0.0142} & \textbf{+0.0234} \\
%     \bottomrule
%     \end{tabular}
%     \vspace{-0.3cm}
%     }%
%   \label{tab:result1}%
% \end{table}%

% % Table generated by Excel2LaTeX
% % The AUC performance (mean$\pm$std) on the public dataset. The Gain means the mean AUC improvement compared with the LightGBM. Underlined results indicate the best baselines over each task. ``*'' indicates that the improvement of the proposed \model~ is statistically significant compared with the best baselines at p-value $<$ 0.05 over paired samples t-test, and ``**'' indicates that the p-value $<$ 0.01.
% \begin{table}[!t]
%   \centering
%   \caption{The AUC performance (mean$\pm$std) on the public dataset.}
%   \vspace{-0.3cm}
%     \setlength{\tabcolsep}{1mm}{
%     \begin{tabular}{cllll}
%     \toprule
%     Model & \click~ AUC & \purchase~ AUC & \multicolumn{2}{c}{Gain} \\
%     \midrule
%     LightGBM & 0.5837$\pm$0.0005 & 0.5870$\pm$0.0038 & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} \\
%     MLP  & 0.6048$\pm$0.0013 & 0.5806$\pm$0.0035 & +0.0211  & -0.0064  \\
%     \midrule
%     ESMM  & 0.6022$\pm$0.0020 & 0.6291$\pm$0.0061 & +0.0185  & +0.0421  \\
%     OMoE  & \underline{0.6049$\pm$0.0020} & 0.6405$\pm$0.0041 & \textbf{+0.0212} & +0.0535  \\
%     MMoE  & 0.6047$\pm$0.0017 & \underline{0.6420$\pm$0.0031} & +0.0210  & +0.0550  \\
%     PLE   & 0.6039$\pm$0.0014 & 0.6417$\pm$0.0013 & +0.0202  & +0.0547  \\
%     AITM  & 0.6043$\pm$0.0016 & \textbf{0.6525$\pm$0.0024**} & +0.0206  & \textbf{+0.0655} \\
%     \bottomrule
%     \end{tabular}
%     \vspace{-0.3cm}
%     }%
%   \label{tab:result2}%
% \end{table}%
\begin{figure*}[!t]
\begin{center}
\includegraphics[width=0.925\linewidth]{activate}
\caption{The t-SNE visualization at different conversion score rankings of the original information $\q_t$, transferred plus original information  $\p_{t-1}+\q_t$  and the information $\z_t$ learned by the \module~ on the \textit{\textbf{activation}} task.}
\label{fig:activate}%
\end{center}
\end{figure*}%

In this subsection, we report the AUC scores and gains of all models on the offline test set. 
As mentioned in Section \ref{sec:main_task}, we only focus on the last two main end-to-end conversion tasks on the industrial dataset. 
The results of \credit~ AUC and \activate~ AUC are shown in Table \ref{tab:result12}.
From these results, we have the following insightful observations:
\begin{itemize}
    \item The MLP obtains $0.0018$ and $0.0066$ AUC gains on two tasks, respectively, compared with the tree-based model LightGBM, which indicates the fitting ability of neural network models on large-scale datasets.
    \item Compared with the single-task models LightGBM and MLP, the multi-task models ESMM, OMoE, MMoE, PLE and AITM obtain more gains by introducing the multi-task information in the neural networks.
    \item The Probability-Transfer pattern-based ESMM achieves a relatively small improvement due to only simple probability information is transferred between adjacent tasks.
    \item The Expert-Bottom pattern-based models obtain further performance improvement by controlling the shared information among different tasks. However, neither of the one-gate and multi-gate models is a clear winner on this dataset.
    \item The PLE obtains the best performance among these baselines on the two tasks via separating task-shared experts and task-specific experts explicitly.
    \item Our \model~achieves significant improvement compared with various state-of-the-art baseline models, which shows the \module~module is effective and could bring more gains on sequential dependence tasks.
\end{itemize}
The results on the public dataset are also shown in Table \ref{tab:result12}.
From these results, we have the following  findings, which are not the same as above:
\begin{itemize}
    \item Serious class imbalance on the \purchase~ task (the proportion of positive samples is $0.02\%$ as shown in Table \ref{tab:dataset}) leads to the poor performance of the two single-task models, i.e., the LightGBM and MLP.
    \item The MLP obtains similar performance improvement compared with multi-task models on the \click~ task. In other words, the multi-task models seem to have no significant improvement on the \click~ task. This may be because there are only two tasks in this dataset, and no other task can provide more information before the \click~ task. $3.89\%$ positive samples in the \click~ task are relatively abundant as shown in Table \ref{tab:dataset}.
    \item The Expert-Bottom pattern shows better performance than the Probability-Transfer pattern on the \purchase~ task with serious class imbalance. Besides, our \model~ can explicitly use the rich positive sample information of the former \click~ task to alleviate the class imbalance of the current \purchase~ task and achieve the best performance. On the other hand, it also shows the generalization ability of the proposed \model.
\end{itemize}

\subsubsection{\textbf{Online Results}}

% Table generated by Excel2LaTeX from sheet '大数据集'
\begin{table}[!t]
  \centering
  \caption{Online A/B test results.}
    \setlength{\tabcolsep}{5mm}{\begin{tabular}{ccc}
    \toprule
    \multirow{2}[2]{*}{Model} & \multicolumn{2}{c}{Gain} \\
          & \credit~ & \activate~ \\
    \midrule
    MLP vs LightGBM & +16.95\% & +17.55\% \\
    AITM vs MLP & +25.00\% & +42.11\% \\
    \bottomrule
    \end{tabular}
    }%
  \label{tab:result_online}%
\end{table}%

The proposed framework is trained offline and regularly updated. 
The pre-trained model is deployed in Meituan app by the TF Serving\footnote{https://github.com/tensorflow/serving}, to real-timely show a banner to the audience with a high end-to-end \credit~ or \activate~ conversion rate for Meituan Co-Branded Credit Cards.
Due to business competition, user experience, and delayed feedback (T+14) of the \activate~ task, we can not deploy all models to the online system. 
With the development of our business, we have successively deployed LightGBM, MLP, and AITM to the online system.
These models serve tens of millions of traffic every day.
A/B test is carried out for every two models with the same traffic for two consecutive weeks (It takes four weeks for all feedback to be received for every two models).
The online A/B test results are shown in Table \ref{tab:result_online}.
Compared with LightGBM, the \impression~ $\rightarrow$ \credit~ conversion rate of MLP increases by $16.95\%$ and the \impression~ $\rightarrow$ \activate~ conversion rate increases by $17.55\%$.
The \model~ further increases the \impression~$\rightarrow$\credit~ and \impression~ $\rightarrow$ \activate~ 
conversion rate by $25.00\%$, $42.11\%$ compared with MLP, respectively. 
Now, the \model~ has provided real-time prediction for all traffic in our system.

Besides, our system is computationally efficient, and the TP999, TP9999 of the real-time prediction is less than 20ms, 30ms in the system every day, respectively, which can meet the requirement of real-time solutions.

\begin{figure*}[!t]
\begin{center}
\includegraphics[width=0.95\linewidth]{params}
\caption{The mean AUC performance in different experiment settings, the shaded part represents the standard deviation. (a) The impact of the embedding dimension $d$. (b) The impact of the strength $\alpha$ of the \constraint. (c) The impact of the proportion $\lambda$ of positive samples. (d) Ablation Study of the number $T$ of tasks.}
\label{fig:params}%
\end{center}
\end{figure*}%
\begin{figure}[!t]
\begin{center}
\includegraphics[width=0.95\linewidth]{weight}
\caption{The mean weight $w_u$ of the transferred information $\p_{t-1}$ over different conversion stages (00/10/11) at different logloss rankings, the shaded part represents the standard deviation. (a) The tasks \textit{\textbf{application}}~$\rightarrow$~\textit{\textbf{approval}}. (b) The tasks \textit{\textbf{approval}~}$\rightarrow$~\textit{\textbf{activation}}.}
\label{fig:weight}%
\end{center}
\end{figure}%
\subsection{Ablation Study}\label{sub:ablation}
% \begin{figure*}[!t]
% \begin{center}
% \includegraphics[width=\linewidth]{credit}
% \caption{}
% \label{fig:credit}%
% \end{center}
% \end{figure*}%

In this subsection, we perform the ablation study of the \module~ module and the number of the tasks.

Firstly, we randomly sample $500$ \activate~ positive and negative samples in the test set, respectively.
The \activate~ prediction scores of positive samples are ranked in descending order, while those of negative samples are in ascending order.
We plot the original information $\q_t$, transferred plus original information $\p_{t-1}+\q_t$  and the information $\z_t$ learned by the \module~ on the \activate~ task in Figure \ref{fig:activate} via the t-SNE (t-distributed Stochastic Neighbor Embedding \cite{tsne2008}).
From the visualization, we can obtain the following inspiring observations (Similar results can also be observed in the \credit~ task, we list it in the appendix due to the space limitation):
\begin{itemize}
    \item When the prediction scores of the \model~ are very confident (see the Top $0\%-50\%$ in Figure \ref{fig:activate}), the three components (i.e., the Original, Transferred+Original, and AIT) can accurately identify positive and negative samples.
    \item With the confidence of the prediction scores of the \model~ decreases (see the Top $50\%-100\%$ in Figure \ref{fig:activate}), it is difficult to identify positive and negative samples only using the original information. The transferred plus original information improves the performance compared with only the original information, which indicates that information transfer could improve the performance of tasks with sequential dependence in multi-task learning.
    \item The \module~ module could adaptively learn what and how much information to transfer among audience multi-step conversions via the multi-task framework,
    so the \module~ further improves the performance compared with the transferred plus original information under low confidence.
\end{itemize}
Besides, we study the impact of the number of tasks as shown in Figure \ref{fig:params} (d). We perform the experiments over tasks \activate~ (\credit), \credit~ $\rightarrow$ \activate, \apply~ $\rightarrow$ \credit~ $\rightarrow$ \activate, $click~\\\rightarrow$ \apply~ $\rightarrow$ \credit~ $\rightarrow$ \activate, respectively. More tasks with more positive sample information and transferred information greatly improve the performance.

\subsection{Case Study}
In order to understand how much information the \module~ module transfers for different conversion stages, we extract the weight $w_u$ in Equation (\ref{eqt:weight}) of the transferred information $\p_{t-1}$ and show it in Figure \ref{fig:weight}.
We first randomly sample $40,000$ test samples.
In Figure \ref{fig:weight} (a), we divide the samples into three groups according to the \apply~ and \credit~ labels of $00/10/11$, and rank the top $500$ samples in each group according to the logloss of each sample in ascending order. Figure \ref{fig:weight} (b) is the same except for the tasks are \credit~ and \activate.
From Figure \ref{fig:weight}, we have the following interesting findings:
\begin{itemize}
    \item Because when the label of the former task is 0, the label of the latter task must also be 0, we can see that at this time the former task transfers very strong information to the latter task (the weight is close to 1 of the red lines in Figure \ref{fig:weight}).
    \item When the label of the former task is 1, the label of the latter task is uncertain. 
    When the label of the latter task is 1, there is little information is transferred from the former task (the green lines in Figure \ref{fig:weight}), which indicates that the latter task mainly identifies positive samples based on the task itself.
    \item When the label of the former task is 1, with the prediction becomes worse (the logloss rankings from 0\%-25\% to 75\%-100\%), the weight of the transferred information gradually increases (the blue and green lines in Figure \ref{fig:weight}), which indicates that the prediction result of the latter task is misled by the former task.
\end{itemize}
From the above results, we could see that the \module~ module can learn how much information to transfer between two adjacent tasks.

\subsection{Hype-parameter Study}
In order to study the impact of hype-parameters and the stability on the performance of the \model, we perform the hyper-parameter study.

Firstly, considering the embedding dimension $d$, we vary the embedding dimension as $[1,5,10,16,32,64,128]$, the results are shown in Figure \ref{fig:params} (a).
We can see that the performance of the \model~ is not very sensitive to the embedding dimension.
The embedding dimension is related to the complexity and capability of the model. Usually, smaller embedding dimension may fit the data distribution insufficiently, especially if the numbers of samples and features are large. While a larger embedding dimension increases the complexity of the model and requires more samples and features to fit, a proper embedding dimension can achieve the best performance \cite{bistddp2019modelling}. Making a trade-off between model complexity and capability, we finally set $d = 5$ as the embedding dimension in all experiments.

Secondly, we study the impact of the strength $\alpha$ of the \constraint~ as shown in Figure \ref{fig:params} (b). 
There are performance fluctuations (the seesaw phenomenon) among four different tasks. However, the \constraint~ brings the improvement of the overall performance. We finally set $\alpha = 0.6$ as the weight in all the experiments.

Thirdly, we study the impact of the proportion $\lambda$ of positive samples in the industrial dataset.
We downsample the \activate~ negative samples to keep the proportion $\lambda$ of positive samples to be $[0.025\%,0.05\%,0.125\%,0.25\%,$ $0.5\%,1\%,2.5\%,5\%]$ in the train set, respectively, and report the AUC performance on the entire test set in Figure \ref{fig:params} (c).
On the one hand, if audiences do not apply for the credit card at present, it does not mean that they will not apply for the card in the future, so we can not use too many negative samples for training.
On the other hand, it can be seen that when $\lambda$ is too large, the performance of the model drops sharply. This is because too much \activate~ negative sample information is lost.
Besides, excessive downsampling of the \activate~ negative samples also leads to the loss of \credit~ positive samples.
We finally downsample the \activate~ negative samples to keep the proportion $\lambda$ of positive samples to be $1\%$. 
This setting is applied to all models.

Combining the performance in Table \ref{tab:result12} and Figure \ref{fig:params}, we can see that even without the best parameters, the \model~ is still superior to other baselines in most cases. 
In other words, the performance of the \model~ stays stable in a large range of values of hyper-parameters and is not very sensitive to the hyper-parameters.

==> KDD21 applied data science track/input/introduction.tex <==
\section{Introduction}\label{introduction}
\begin{figure}[!t]
\begin{center}
\includegraphics[width=0.9\linewidth]{conversion_stages}
\caption{There are five conversion steps with sequential dependence from left to right, and five different conversion stages of audiences from top to bottom. The lower the stage, the more efficient the conversion. In our business, we usually hope audiences to complete the last two stages.}
\label{fig:conversion_stages}%
\end{center}
\end{figure}%

% Customer acquisition management is a set of techniques used to manage customer prospects and inquiries generated by marketing. 
Customer acquisition management can be considered the connection between advertising and customer relationship management to acquire new customers\footnote{https://en.wikipedia.org/wiki/Customer\_acquisition\_management}.
With the explosive growth of e-commerce, continuous and effective customer acquisition has become one of the biggest challenges for real-world large-scale online applications. 

In this paper, we focus on the customer acquisition task with sequential dependence among audience multi-step conversions.
Typically, in the credit card business, the audience multi-step conversion process usually needs to go through \impression~ $\rightarrow$ \click~ $\rightarrow$ \apply~ $\rightarrow$ \credit~ $\rightarrow$ \activate~ steps. These steps are defined as follows:

% \begin{itemize} 
- \bm{\impression}: 
% This step is usually a priori condition for the audience to start the conversion process, and it is usually a passive step for the audience.
In our business, the \impression~
means that the advertising banner is shown to the audience selected according to several ranking metrics, e.g., the Click-Through Rate (CTR).

- \bm{\click}: The \click~ means that the shown banner is clicked by the audience, and redirected to the application page. 

- \bm{\apply}: The \apply~ means that the audience has filled in the application form and click the application button for a credit card.

- \bm{\credit}: The \credit~ means that the credit of the audience has been approved. In our system, this is also a real-time step.

- \bm{\activate}: The \activate~ is delayed feedback, and it means that the audience has activated the credit card within a period of time after \credit. Usually, we consider whether the audience has activated the credit card within 14 days (i.e., activation in T+14). 
The \activate~ feedback label is usually difficult to obtain due to the time-consuming of card mailing and the delayed feedback of audiences, so the class imbalance is more serious.
% \end{itemize}

These conversion steps have sequential dependence, which means that only the former step occurs, the latter step may occur.
Based on this constraint, there are five different conversion stages of audiences as shown in Figure \ref{fig:conversion_stages}. Everything else is illegal. 

In industry and academia, multi-task learning is a typical solution to improve the end-to-end conversion in the audience multi-step conversion task.
Recently, considerable efforts have been done to model task relationships in multi-task learning. 
One idea is to control how Expert modules are shared across all tasks at the bottom of the multi-task model \cite{mmoe2018kdd,cgc2020recsys,mmoe2020seq}, and Tower modules at the top handle each task separately as shown in Figure \ref{fig:model} (a).
However, the Expert-Bottom pattern can only transfer shallow representations among tasks, but in the network close to the output layer, it often contains richer and more useful representations \cite{visual2014visualizing,visual2016convergent}, which have been proved to bring more gains \cite{mmd2014deep}.
Besides, the Expert-Bottom pattern is not specially designed for tasks with sequential dependence, so these models with the Expert-Bottom pattern can not model the sequential dependence explicitly.
Another idea is to transfer probabilities in the output layers of different tasks \cite{esmm2018sigir,npt2019neural,gao2019learning,esm22020sigir} as shown in Figure \ref{fig:model} (b). 
Similarly, the Probability-Transfer pattern can only transfer simple probability information via the scalar product, but richer and more useful representations are ignored in the vector space, which results in a great loss of gains.
If any one of the probabilities is not predicted accurately, multiple tasks will be affected.
Besides, the Probability-Transfer pattern is designed for solving the non-end-to-end post-click conversion rate via training on the entire space to relieve the sample selection bias problem, and these models with Probability-Transfer pattern can not model the sequential dependence well among audience multi-step conversions.
Therefore, a long-standing challenge is how to model the sequential dependence among audience multi-step conversions for improving the end-to-end conversion.

Along this line, we propose an Adaptive Information Transfer  Multi-task (\model) framework to model the sequential dependence among audience multi-step conversions. Specifically, due to the sequential dependence among audience multi-step conversions, the former conversion step (task) can bring useful information to the latter step (task). For example, if an audience has clicked the banner, then he/she may apply for the credit card. Conversely, if an audience doesn't click the banner, he/she certainly will not  apply for the credit card. 
Based on this, different conversion stages of different audiences need to transfer different information from the former step to the latter step, and as mentioned above, the vector space close to the output layer often contains richer and more useful information.
Therefore, we let the model adaptively transfer information in the vector space close to the output layer via the Adaptive Information Transfer (\module) module. 
Another advantage of the \module~module is that it can alleviate the class imbalance of the latter task with the help of the information from the former task, which has richer positive samples.
Also, because of the sequential dependence, the former task should have a higher end-to-end conversion probability than the latter for the same audience.
Therefore, we design a \constraint~ in the loss function.
On the one hand, it makes the model results more satisfy the real production constraint, on the other hand, it provides more accurate end-to-end conversion identification.
\begin{figure*}[!t]
\begin{center}
\includegraphics[width=0.9\linewidth]{model}
\caption{(a) Expert-Bottom pattern. (b) Probability-Transfer pattern. The $\hat{y}_{o}$ is the non-end-to-end post-click conversion rate and the multi-task loss function only acts on the $\hat{y}_{t-1}$ and $\hat{y}_{t}$ in the original paper. (c) The proposed Adaptive Information Transfer Multi-task (\model) framework. For simplicity, only two adjacent tasks are shown in the figure.}
\label{fig:model}%
\end{center}
\end{figure*}%
To summarize, the contributions of this paper are threefold:
\begin{itemize}
    \item The proposed \module~ module can adaptively learn what and how much information to transfer for different conversion stages of different audiences for improving the performance of multi-task learning with sequential dependence.
    \item Combining the \constraint~ in the loss function, offline experimental results on both industrial and public real-life datasets clearly demonstrate that the proposed framework achieves significantly better performance compared with state-of-the-art baselines.
    \item Online experiments also demonstrate significant improvement compared with existing online models, and the source code of the proposed framework has also been released.
    % \footnote{https://github.com/xidongbo/AITM}.
\end{itemize}



==> KDD21 applied data science track/input/methodology.tex <==
\section{The MTL Ranking System in Meituan app}\label{sec:main_task}
\begin{figure*}[!t]
\begin{center}
\includegraphics[width=0.95\linewidth]{system}
\caption{The MTL Ranking System in Meituan app.}
\label{fig:system}%
\end{center}
\end{figure*}%
In this section, we give an overview of the MTL ranking system in Meituan app.
As shown in Figure \ref{fig:system}, in our credit card business, we model four tasks except for the passive \impression~step. 
Among them, the \credit~and \activate~are the main tasks, and the \click~and \apply~are the auxiliary tasks. 
That is because if the audience has only completed the \click~ and \apply~ steps, but the \credit~ step has not been completed, then it will cause a waste of resources (e.g., the computing and traffic resources). 
Because different audiences have different values to different businesses, the traffic that is useless to the credit card business may be useful to other businesses.
For this kind of audience, we might as well give the traffic to other businesses that may promote the audience conversion.
Therefore, we mainly focus on the last two end-to-end conversion tasks, i.e., \impression $\rightarrow$ \credit~and \impression $\rightarrow$ \activate.
Besides, because the last two tasks have fewer positive samples and the \activate~is delayed feedback, the first two auxiliary tasks with more positive samples can alleviate the class imbalance problem via the Adaptive Information Transfer module.

Meituan Co-Branded Credit Cards are issued in cooperation with different banks, and different banks are in different stages of business development, so they have different requirements for the \credit~and \activate. 
Start-up banks often want to issue more credit cards to quickly occupy the market, while mature banks want to increase the activation rate to achieve rapid profits.
Therefore, there is a selector in our system to output different conversion objectives for different banks.
The multi-task framework can deal with different business requirements well.

Besides, because different businesses in Meituan all need the traffic to acquire customers for their own business, and the sensitivities of different audiences to different businesses are different, so we can not simply divide the traffic into different businesses. 
We need a ranking mechanism to maximize the overall gain.
The multi-business ranking system ranks the different business scores according to the Equation:
\begin{eqnarray}
score = weight\times\hat{y},
\end{eqnarray}
where $\hat{y}$ is the predicted conversion probability for each business, and the $weight$ includes the value of the audience itself, the value of the business itself, and the value of the audience to the business.
The business banner with the highest score is shown to the audience.

\section{Methodology}
In this section, we first formulate the problem, then
we present the details of the proposed framework \model~ as shown in Figure \ref{fig:model} (c).

\subsection{Problem Formulation}
Given the input feature vector $\x$, assuming the audience needs $T$ steps to complete the final conversion after \impression~ (In Figure \ref{fig:conversion_stages}, $T=4$). In each conversion step $t$, if the audience completes the conversion step, the label $y_t$ is $1$, otherwise it is $0$. The sequential dependence means that $y_1\geq y_2\geq\cdots\geq y_T$ ($y_t\in \{0, 1\}, t = 1, 2, \cdots, T$). 
The multi-task framework needs to predict the end-to-end conversion probability $\hat{y}_t$ of each conversion step $t$ based on the input features $\x$:
\begin{equation}
\hat{y}_t = p(y_1=1,y_2=1,\cdots,y_t=1|\x).
\end{equation}%


\subsection{Adaptive Information Transfer Multi-task (\model) framework}
As shown in Figure \ref{fig:model} (c), given the input feature vector $\x$, 
we embed each entry $x_i$ ($x_i\in\x$, $1\leq i\leq|\x|$) to a low dimension dense vector representation $\v_i\in\setR^d$, where $d$ is the dimension of embedding vectors. The output of the Shared Embedding module is the concatenation of all embedding vectors: 
\begin{eqnarray}
\v = [\v_1;\v_2;\cdots;\v_{|\x|}],
\end{eqnarray}
where $[\cdot;\cdot]$ denotes the concatenation of two vectors.
By sharing the same embedding vectors among all tasks, on the one hand, the framework could learn the embedding vectors with rich positive samples of the former tasks to share information and alleviate the class imbalance of the latter tasks, and reduce the model parameters on the other hand.

Given $T$ tasks, the output of the Tower of each task $t (1\leq t\leq T)$ is defined as:
\begin{eqnarray}
\q_t=f_t(\v),
\end{eqnarray}
where the $f_t(\cdot)$ function is the Tower, $\q_t\in\setR^k$ and $k$ is the output dimension of the Tower. 
It should be mentioned that designing a different Tower is not the focus of this paper as we aim at designing an Adaptive Information Transfer module to model the sequential dependence.
In fact, our approach is a general framework, and any advanced models (e.g., NFM \cite{he2017nfm}, DeepFM \cite{guo2017deepfm}, AFM \cite{xiao2017afm}, and even the sequence models NHFM \cite{nhfm2020neural}, DIFM \cite{difm2021modeling}) can be easily integrated into our framework to act as the Tower, making the proposed \model~general and flexible.

For two adjacent tasks $t-1$ and $t$, the output of the AIT module of the task $t$ is computed as:
\begin{eqnarray}
\z_t&=&AIT(\p_{t-1}, \q_t), \\
where~\p_{t-1}&=&g_{t-1}(\z_{t-1}),
\end{eqnarray}
$\z_{t-1}\in\setR^k$ is the output of the AIT module of the task $t-1$, $g_{t-1}(\cdot)$ is the function to learn what information to transfer between the tasks $t-1$ and $t$, and $\p_{t-1}\in\setR^k$ is the learned transfer information.

The AIT module is designed to adaptively allocate the weights of the transferred information $\p_{t-1}$ and original information $\q_t$:
\begin{eqnarray} 
\z_t&=&\sum_{\u\in\{\p_{t-1},\q_t\}}w_uh_1(\u), \label{eqt:att}
\end{eqnarray}
where $w_u$ is the weight which is formulated as:
\begin{eqnarray} 
w_u=\frac{exp(\hat{w}_u)}{\sum_{u}exp(\hat{w}_u)},~~
\hat{w}_u=\frac{<h_2(\u),h_3(\u)>}{\sqrt{k}},
\label{eqt:weight}
\end{eqnarray}
where $<\cdot~, \cdot>$ represents the dot product.
$h_1(\cdot)$, $h_2(\cdot)$, and $h_3(\cdot)$ represent the feed-forward networks to project the input information to one new vector representation. There are lots of ways to design $h_1(\cdot)$, $h_2(\cdot)$, and $h_3(\cdot)$. In this paper, we use a simple single-layer MLP (Multi-Layer Perceptron) \cite{gardner1998mlp} as $h_1(\cdot)$, $h_2(\cdot)$, and $h_3(\cdot)$.
The idea of this kind of attention mechanism is similar to self-attention \cite{self2017attention}, the $h_1(\cdot)$, $h_2(\cdot)$ and, $h_3(\cdot)$ first learn Value, Query, Key from the same input $\u$, respectively. Then, we compute the similarity between Query ($h_2(\cdot)$) and Key ($h_3(\cdot)$) according to Equation (\ref{eqt:weight}). Finally, the Value ($h_1(\cdot)$) is weighted via the similarity according to Equation \ref{eqt:att}. 
This kind of attention mechanism has been proved to be more effective in the previous works \cite{nhfm2020neural,www2020modeling,difm2021modeling}. 

For the first task without the former task, the out of the AIT module is initialized to:
\begin{eqnarray} 
\z_1=\q_1.
\end{eqnarray}

The prediction probability of each task $t$ is:
\begin{eqnarray} 
\hat{y}_t=sigmoid(MLP(\z_t)),
% \sigma(x)&=&\frac{1}{1+e^{-x}}\in[0,1]\\
% tanh(x)&=&\frac{e^x-e^{-x}}{e^x+e^{-1}}\in[-1,1]\\
% relu(x)&=&max(0,x)\in[0,+\infty)\\
% softmax(x)&=&\frac{e^x}{\sum_{x'}e^{x'}}\in[0,1]
\end{eqnarray}
where the MLP is used to project the $\z_t$ to the output space.

\subsection{\constraint~ and Joint Opratortimization for MTL}
For classification tasks, we need to minimize the \textit{cross-entropy} loss of all tasks:
\begin{equation}
\small{
\L_{ce}(\theta)=-\frac{1}{N}\sum_{t=1}^{T}\sum^N_{(\x,y_t)\in\D}(\left(y_t\log\hat{y}_t+(1-y_t)\log(1-\hat{y}_t)\right)},
\end{equation}
where $N$ is the number of samples in the entire sample space $\D$, $y_t$ is the label of the $t$-th task and $\theta$ is the parameter set in the MTL framework.

Besides, because of the sequential dependence, the former task should have a higher end-to-end conversion probability than the latter for the same audience, i.e., $\hat{y}_{t-1}\geq\hat{y}_t$.
We design a \constraint~ to minimize the following objective. On the one hand, it makes the model results more satisfy the real production constraint, on the other hand, it provides more accurate end-to-end conversion identification: 
\begin{equation}
\L_{lc}(\theta)=\frac{1}{N}\sum_{t=2}^{T}\sum^N_{\x\in\D}max(\hat{y}_t-\hat{y}_{t-1},0).
\end{equation}%
If $\hat{y}_t>\hat{y}_{t-1}$, the $\L_{lc}(\theta)$ will output a positive penalty term, otherwise output 0.

The final loss function $\L(\theta)$ of the \model~ combines the two components to a unified multi-task learning framework:
\begin{equation}
\L(\theta)=\L_{ce}(\theta)+\alpha\L_{lc}(\theta),
\end{equation}%
where $\alpha$ controls the strength of the \constraint~ component.

The framework is implemented using TensorFlow\footnote{https://www.tensorflow.org/} and trained through stochastic gradient descent over shuffled mini-batches with the Adam \cite{adam2015method} update rule.

==> KDD21 applied data science track/input/related_work.tex <==
\section{Related Work}
Multi-task learning (MTL) has led to successes in many applications of machine learning, from natural language processing and speech recognition to computer vision and drug discovery \cite{survey2017overview}.
In this section, we present the main multi-task learning works related to our work in two-fold:
the Expert-Bottom pattern and the Probability-Transfer pattern.

As shown in Figure \ref{fig:model} (a), the main idea of the Expert-Bottom pattern is to control how Expert modules are shared across all tasks at the bottom of the multi-task model \cite{mmoe2018kdd,cgc2020recsys,mmoe2020seq}, and the Tower modules at the top handle each task separately. Since complex problems may contain many sub-problems each requiring different experts \cite{moe22013learning}, some Mixture-of-Experts (MoE) models have been proposed one after another \cite{moe11991adaptive,moe22013learning,moe32017outrageously}. Inspired by the idea, \citeauthor{mmoe2018kdd} introduced the MoE to the multi-task learning and proposed the Multi-gate Mixture-of-Experts (MMoE) \cite{mmoe2018kdd} model by the gating networks assembling the experts for different tasks.  
\citeauthor{mmo22019video} explored a variety of soft-parameter sharing techniques such as MMoE to efficiently optimize for multiple ranking objectives for Video recommendation \cite{mmo22019video}.
\citeauthor{cgc2020recsys} proposed a Progressive Layered Extraction (PLE) \cite{cgc2020recsys} model to separate task-shared experts and task-specific experts explicitly. 
The Mixture of Sequential Experts (MoSE) model \cite{mmoe2020seq} has also been proposed to model sequential user behaviors in multi-task learning.  
However, the top Tower modules, which often contain richer and more useful information, can not help the tasks to improve each other due to there is no information exchange among them.

Another idea to model task relationships in multi-task learning is to transfer probabilities in the output layers of different tasks \cite{esmm2018sigir,npt2019neural,gao2019learning,esm22020sigir} as shown in Figure \ref{fig:model} (b).
\citeauthor{esmm2018sigir} proposed an Entire Space Multi-task Model (ESMM) \cite{esmm2018sigir} to transfer probabilities in the output layers by post-impression click-through rate (CTR) multiplying post-click conversion rate (CVR) equals post-impression click-through$\&$conversion rate (CTCVR). 
Further, more tasks are decomposed for probability transfer in $ESM^2$ \cite{esm22020sigir}.
The Neural Multi-Task Recommendation (NMTR) \cite{npt2019neural,gao2019learning} has also been proposed to extend the Neural Collaborative Filtering (NCF) \cite{ncf2017neural} to multi-task learning and relate the model prediction probability of each task in a cascaded manner.
% However, the Probability-Transfer pattern is designed for solving the non-end-to-end post-click conversion rate via training on the entire space to relieve the sample selection bias problem, and these models with Probability-Transfer pattern can not model the sequential dependence well among audience multi-step conversions.
However, as mentioned in Section \ref{introduction}, the Probability-Transfer pattern can only transfer simple probability information via the scalar product, but richer and more useful representations are ignored in the vector space, which results in a great loss. 
Besides, if any one of the probabilities is not predicted accurately, multiple tasks will be affected.

Other efforts have also utilized the tensor factorization \cite{tensor2017deep}, tensor normal priors \cite{tensor2017priors}, attention mechanism \cite{attention12019end,attention2019z}, and so on to solve the multi-task learning.
Nevertheless, these above efforts are not specially designed for tasks with sequential dependence, and they can not model the sequential dependence well among audience multi-step conversions.

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.75.  \country is now obligatory for addresses.
	       Added \AtBeginMaketitle

Version 1.76.  Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.77.  Changed the way to typset multiple affiliations (Christoph Sommer)
